Diameter of P.A. random graphs with edge-step functions

In this work we prove general bounds for the diameter of random graphs generated by a preferential attachment model whose parameter is a function $f:\mathbb{N}\to[0,1]$ that drives the asymptotic proportion between the numbers of vertices and edges. These results are sharp when $f$ is a \textit{regularly varying function at infinity} with strictly negative index of regular variation~$-\gamma$. For this particular class, we prove a characterization for the diameter that depends only on~$-\gamma$. More specifically, we prove that the diameter of such graphs is of order $1/\gamma$ with high probability, although its vertex set order goes to infinity polynomially. Sharp results for the diameter for a wide class of \textit{slowly varying functions} are also obtained.

==> prooflargecliques.tex <==
%! TEX root = Diameter-Edge_step.tex
Given~$\delta>0$ sufficiently small, let $\varepsilon,p=\delta/6$ so that
\begin{equation*}
\alpha=\alpha(p,\varepsilon):=\frac{1-p}{2-p}(1-\varepsilon)>\frac{1}{2}\left(1-\frac{\delta}{2}\right).
\end{equation*}
In the proof of Theorem~$1$ of~\cite{ARS17} one uses Theorem~$2$ of~\cite{ARS17} to show that there exist a fixed integer~$m=m(\e,p)>0$ and a small number $\varepsilon'\in(0,\alpha)$ with the following property: if one divides the set of vertices born between times~$t^{\varepsilon'}$ and~$t^\alpha$ into disjoint subsets of~$m$ vertices born \emph{consecutively}, then with high probability (at least $1$ minus a polynomial function of~$t$) one can choose a vertex from each of these subsets in such a way that the subgraph induced by the set of chosen vertices is a complete subgraph of~$G_t(\mathrm{cons}_p)$. 

Having the above in mind and letting $m$ be the auxiliary $m$ that appears in proof of Theorem~1 of \cite{ARS17}, define the following event
\begin{equation}
A_{p, \varepsilon', m, k} := \left \lbrace 
\begin{array}{c}
\exists \{t_1, \cdots, t_k\} \subset [t] \text{ such that } t_j \in (t^{\varepsilon'}+(j-1)m, t^{\varepsilon'}+jm] \\
\text{and }v_{t_j} \leftrightarrow v_{t_i} \textit{ in }G_t(\mathrm{cons}_p) \text{ for all } i,j \in [k]
\end{array}
\right \rbrace.
\end{equation}
In the context of the doubly labeled tree process, the event $A_{p, \varepsilon', m, k}$ says that we may find~$k$ vertices of $\cal{T}_t$ with the property that the $j$-th vertex $v_{t_j}$ was added by the doubly-labeled tree process sometime in the interval~$(t^{\varepsilon'}+(j-1)m, t^{\varepsilon'}+jm]$ and its~$U_{t_j}$-label is less than~$p$. Moreover, when we apply~$\mathrm{cons}_p$ on $\cal{T}_t$ in the event~$A_{p, \varepsilon', m, k}$, all these~$k$ vertices form a complete graph in the resulting graph $G_t(\mathrm{cons}_p)$. Theorem~$1$ of~\cite{ARS17} states that setting $k = t^{\alpha} - t^{\varepsilon'}$, the event~$A_{p, \varepsilon', m, k}$ occurs with probability at least $1-t^{-\eta}$, for some positive small $\eta$ depending on $p$, which, in our case, is a function of $\delta$. Thus, for $t$ large enough, we may simply use that
\begin{equation}\label{ineq:probA}
\Pd\left(A_{p, \varepsilon', m, t^{\alpha}}\right) \ge 1 - \frac{1}{\log t},
\end{equation}
this bound will be useful for the proof of Corollary~\ref{cor:cliquesRV}. This is why we are exchanging a polynomial decay by a $\log$ one, to get rid off the dependency on $\delta$ and consequently simplify latter arguments.

Now, let $t$ be large enough so that $f(t^{\varepsilon'}) < p$. This is possible since $f$ decreases to zero. Also notice that if $u$ and $v$ are vertices of $G_t(f)$ added after time $t^{\varepsilon'}$ and are connected in~$G_t(\mathrm{cons}_p)$, then they are connected in $G_t(f)$ as well. Moreover, since $f$ is non-increasing and the $U$-labels are assigned independently and according to a uniform distribution on $[0,1]$, we have for all $j \le k$
\begin{equation}
\Pd \left( U_{t_j} \le f(t_j) \; \middle | \; A_{p, \varepsilon', m, k} \right) \ge p^{-1}f(t^{\varepsilon'}+jm).
\end{equation}
Setting $k= (t^{\alpha} - t^{\varepsilon'})/m$ and using that $f$ is non-increasing, we have that
\begin{equation}
m\sum_{j=0}^kf(t^{\varepsilon'}+jm) \ge F(t^{\alpha}) -F(t^{\varepsilon'}+m) \ge F(t^{\a})/2
\end{equation}
for large enough $t$. 

By the independence of the $U$-labels, it follows that conditioned on $A_{p, \varepsilon', m, k}$, the random variable that counts how many vertices of the clique in $G_t(\mathrm{cons}_p)$ remain vertices of $G_t(f)$ as well is a sum of $k$ independent random variables taking values on $\{0,1\}$ and whose expected value is greater than $F(t^{\a})/2mp$. Finally, by Chernoff bounds, this random variable is at least half its expected value with probability at least $1-\exp\{-F(t^{\alpha})/16mp\}$. This and (\ref{ineq:probA}) gives us that there exists a constant $C_{\delta}$ such that
\begin{equation}\label{ineq:probclique}
\Pd\left( \nexists K_n \subset G_t(f), \textit{ such that }n \ge C_{\delta}F ( t^{\frac{1-\delta}{2}} )\right) \le  \frac{1}{\log t} + e^{-F(t^{\alpha})/16mp},
\end{equation}
which proves the Theorem.

==> treeprocess.tex <==
%!TEX root = ms.tex
In this section we introduce a stochastic process~$\{\mathcal{T}_t\}_{t\geq 1}$ that provides a grand coupling between the random graphs~$\{G_t(f)\}_{t\geq 1}$ for every edge-step function~$f$.

The process $\{\mathcal{T}_t\}_{t\geq 1}$ is essentially a realization of the Barab\'asi-Albert random tree where each vertex has two labels: an earlier vertex chosen according to the preferential attachment rule and an independent uniform random variable. The label consisting in the earlier vertex can be seen as a ``ghost directed edge'', we later use these random labels to collapse subsets of vertices into a single vertex in order to obtain a graph with the same distribution as $G_t(f)$ for any prescribed function~$f:\N\to[0,1]$. 

We begin our process with a graph~$\mathcal{T}_1$ consisting as usual in a single vertex and a single loop connecting said vertex to itself. We then inductively construct the labeled graph~$\mathcal{T}_{t+1}$ from~$\mathcal{T}_t$ in the following way:
\begin{figure}[ht]
\centering
\includegraphics[scale = .63]{gtildedef}
\vspace{0.2cm}
\caption{A sample of the process~$\{\mathcal{T}_t\}_{t\geq 1}$ up to time~$6$ without the uniform labels. The dashed lines indicate the label~$\ell(v_j)$ taken by each vertex~$v_j$.}
\label{f:gtildedef}
\end{figure}
\begin{itemize}
\item [(i)] We add to~$\mathcal{T}_t$ a vertex~$v_{t+1}$;

\item [(ii)] We tag~$v_{t+1}$ with a random label~$\ell(v_{t+1})$ chosen from the set~$V(\mathcal{T}_t)$ with the preferential attachment rule, that is, with probability of choosing~$u\in V(\mathcal{T}_t)$ proportional to the degree of~$u$ in~$\mathcal{T}_t$;

\item [(iii)] Independently from the step above, we add an edge~$\{w,v_{t+1}\}$ to~$E(\mathcal{T}_t)$ where~$w\in V(\mathcal{T}_t)$ is also randomly chosen according to the preferential attachment rule, see Figure~\ref{f:gtildedef}.
\end{itemize}
We then finish the construction by tagging each vertex~$v_j\in V(\mathcal{T}_t)$ with a second label consisting in an independent random variable~$U_j$ with uniform distribution on the interval~$[0,1]$, as shown in Figure~\ref{f:gcaldef}. We note that only the actual edges contribute to the degree taken in consideration in the preferential attachment rule, the tags are not considered.
\begin{figure}[ht]
\centering
\includegraphics[scale = .7]{gcaldef}
\vspace{0.2cm}
\caption{The graph~$\mathcal{T}_6$, now each vertex receives an independent uniform random variable.}
\label{f:gcaldef}
\end{figure}

We now make precise the notation $f(\cal{T}_t)$ which indicates that an edge-step function $f$ may also be seen as a function that maps a doubly-labeled tree to a (multi)graph. Our goal is to define this map in such way that $f(\mathcal{T}_t) \stackrel{d}{=} G_t(f)$.

In order to do so, let us fix such a function~$f$. Given~$v_j\in V(\mathcal{T}_t)$, we compare~$U_j$ to~$f(j)$. If~$U_j\le f(j)$, we do nothing. Otherwise, we collapse~$v_j$ onto its label~$\ell(v_j)$, that is, we consider the set~$\{v_j,\ell(v_j)\}$ to be a single vertex with the same labels as~$\ell(v_j)$. We then update the label of all vertices~$v$ such that~$\ell(v)=v_j$ to~$\{v_j,\ell(v_j)\}$. This procedure is associative in the sense that the order of the vertices on which we perform this operation does not affect the final resulting graph, as long as we perform it for all the vertices of~$\mathcal{T}_t$. We let then $f(\cal{T}_t)$ be the (multi)graph obtained when this procedure has run over all the $t$ vertices of $\cal{T}_t$. We refer to Figure~\ref{f:gfcoupdef} as an illustration of the final outcome. 

In the next proposition we prove that $f(\cal{T}_t)$ is indeed distributed as $G_t(f)$. 
\begin{figure}[ht]
\centering
\includegraphics[scale = .7]{gfcoupdef}
\vspace{0.2cm}
\caption{The figure shows how one can sample the distribution of~$G_6(f)$ using the labeled graph~$\mathcal{T}_6$.}
\label{f:gfcoupdef}
\end{figure}
\begin{proposition}
\label{prop:gcoupling}
Let~$\cal{T}_t$ be the doubly-labeled tree above defined and $f$ an edge-step function. Then,
\[
f(\mathcal{T}_t) \stackrel{d}{=} G_t(f).
\]
\end{proposition}
\begin{proof}
We first observe that the associativity of the collapsing operation and the independence of the sequence $(U_j)_{j\geq 1}$ from the previous operations imply that we can glue together the vertex $v_{t+1}$ to $\ell(v_{t+1})$ whenever $U_{t+1}>f(t+1)$ right after we complete step~(iii) of the above construction by induction. The resulting graph has either a new vertex~$v_{t+1}$ with an edge~$\{w(v_{t+1}),v_{t+1}\}$ or an edge~$\{w(v_{t+1}),\ell(v_{t+1})\}$ with the exact same probability distribution as the~$(t+1)$-th step in the construction of the graph~$(G_t(f))_{t\geq 1}$. By induction, both random graphs have the same distribution.
\end{proof}
In the light of the above discussion and Proposition~\ref{prop:gcoupling}, from now on, we will tacitly assume that all processes $\{G_t(f)\}_{t\ge 1}$ for all edge-step functions are on the same probability space.

A straightforward consequence of Proposition~\ref{prop:gcoupling} is Proposition~\ref{t:dtv} which roughly speaking states that edge-step functions close to each other generate essentially the same processes. Once we have the machinery provided by Proposition~\ref{prop:gcoupling}, the proof of this fact becomes a simple application of the union bound.
\begin{proof}[Proof of Proposition~\ref{t:dtv}] Fixed two edge-step functions $f$ and $h$, by Proposition~\ref{prop:gcoupling} we have that
	\begin{equation}
	\mathrm{Law}(\{G_t(f)\}_{t\geq 1}) = \mathrm{Law}(\{f(\cal{T}_t)\}_{t\geq 1}).
	\end{equation}
Thus
	\begin{equation}
	\begin{split}
	\dist_{TV}\left(\mathrm{Law}(\{G_t(f)\}_{t\geq 1}),\mathrm{Law}(\{G_t(h)\}_{t\geq 1})\right)
	&\leq\Pd\left( \{f(\cal{T}_t)\}_{t\geq 1} \neq \{h(\cal{T}_t)\}_{t\geq 1}     \right)
	\\
	&\leq \sum_{i=1}^\infty \Pd\left(    U_i   \in (f(i)\wedge h(i),f(i)\vee h(i)  )  \right)
	\\
	&=
	\sum_{i=1}^\infty | f (i)- g (i)|
	\end{split}
	\end{equation}
	and the above equation immediately implies~\eqref{eq:dtv2}.
\end{proof}
The next step is to use the coupling provided by the auxiliary process $\{\cal{T}_t\}_{t \ge 1}$ to compare graph observable of graphs generated by different edge-step functions. This method will allow us to transport results we have obtained for a fixed $f$ to other edge-step functions by comparing them with $f$. To do this we introduce the notion of \textit{increasing (decreasing)} graph observable.
\begin{definition}[Monotone graph observable]\label{def:graphobs} We say that a (multi)graph observable $\zeta$ is \textit{increasing} if, given two edge-step functions $f$ and $h$, we have that 
	\begin{equation}\label{eq:incrob}
		f(s) \le h(s), \forall s \le t \implies	\zeta(f(\cal{T}_t)) \le \zeta(h(\cal{T}_t)) \; \textit{a.s.}
	\end{equation}
When the second inequality in (\ref{eq:incrob}) holds with ``$\ge$", we say $\zeta$ is decreasing.
\end{definition}
A first example of an increasing observable is the total number of vertices. Indeed, since every vertex~$v_j$ of $\mathcal{T}_t$ remains preserved under $f$ whenever its $U_j$ label is less than $f(j)$, it follows that every $f$-preserved $v_j$ is $h$-preserved as well whenever~$f \leq h$.

The next proposition states that the maximum degree is a decreasing observable whereas the diameter, in which we are interested in, is an increasing one.
\begin{proposition}\label{p:diammaxdegProp} Let $f$ and $h$ be two edge-step functions satisfying the relation $f(s)\le h(s)$ for all $s \in (1, \infty)$. Then,
\begin{enumerate}[(a)]
	\item the maximum degree is a \emph{decreasing }graph observable. More precisely, if we let $D_{\textit{max}}(G)$ denote the maximum degree of a (multi)graph $G$, then
	\[
	\Pd \left(\forall t \in \N, \; D_{\textit{max}}(G_t(f)) \ge D_{\textit{max}}(G_t(h))\right) = 1;
	\]
	\item the diameter is an \emph{increasing }graph observable. More precisely,
	\[
	\Pd \left(\forall t \in \N, \; \diam(G_t(f)) \le \diam(G_t(h))\right) = 1
	\]
\end{enumerate}

\end{proposition}
\begin{proof} The proofs follow from an analysis of the action of $f$ over $\cal{T}_t$.

\noindent \underline{Proof of part (a):} We first point out that if $v_s$ is a vertex of $\cal{T}_t$ whose $U_s$-label is less than~$f(s)$, then
\begin{equation}
D_{G_t(f)}(v_s) \ge D_{G_t(h)}(v_s).
\end{equation}
To see why the above inequality is true, notice that the degree of $v_s$ in $G_t(f)$ is the total number of solid edges (see Figure~\ref{f:gcaldef}) incident on $v_s$ in $\cal{T}_t$ plus the total number of vertices whose $\ell$-label points to $v_s$ and whose $U$-label is greater than $f$. Formally,
\begin{equation}
D_{G_t(f)}(v_s) = \sum_{r=1}^{t}\mathbb{1}\left\lbrace v_r \to v_s\text{ in }\cal{T}_t \right \rbrace + \mathbb{1}\left\lbrace \ell(v_r) = v_s, U_r \ge f(r) \right \rbrace.
\end{equation}
The contribution of the first term in the RHS of the above identity remains stable under $f$ and $h$, however, since $f(r)\le h(r)$ for all $r\le t$, we automatically have
\[
\mathbb{1}\left\lbrace \ell(v_r) = v_s, U_r \ge f(r) \right \rbrace \ge \mathbb{1}\left\lbrace \ell(v_r) = v_s, U_r \ge h(r) \right \rbrace,
\]
which implies that $D_{G_t(f)}(v_s) \ge D_{G_t(h)}(v_s)$. 

To finish the proof of this part, notice that, if $v_s$ is truly a vertex in $G_t(h)$ but is glued to its $\ell$-label under $f$, this operation just increases the maximum degree in the sense that the degree of $\ell(v_s)$ inherits all the contributions of $v_s$. Thus, if $v_{\textit{max}}$ is a vertex that achieves $D_{\textit{max}}(G_t(h))$, then if $v_{\textit{max}}$ is also a vertex of $G_t(f)$ by the above discussion, its degree is at least $D_{\textit{max}}(G_t(h))$. On the other hand, if it is identified to $\ell(v_{\textit{max}})$, then the degree of $\ell(v_{\textit{max}})$ is also at least the maximum degree of $G_t(h)$.



\noindent \underline{Proof of part (b):} Observe that if $u$ and $w$ are vertices whose $U$-label is less than $f$ and such that $u \leftrightarrow w$ in $G_t(f)$, then $u$ and $w$ are possibly not connected by a single edge in $G_t(h)$, in other words, if $\dist_{G_t(f)}(u,w) = 1$ then $\dist_{G_t(h)}(u,w) \ge 1$. Therefore, if $v_0 =u, v_1, \cdots, v_k = w$ is a minimal path in $G_t(f)$, by the previous observation, this path induces a path in $G_t(h)$ whose length is equal to or greater than $k$.

On the other hand, if $u=v_0 , v_1, \cdots, v_k = w$ is a path realizing the minimal distance between~$u$ and~$w$, in $G_t(h)$ we have that this path induces another path in $G_t(f)$ of same length or less. To see this, just notice that, if $U_j > f(j)$ and $\ell(v_j)$ points to a vertex outside the path for some $j \in \{2,3,\cdots,k-1\}$, then, after identifying $v_j$ to its $\ell$-label, this operation does not increase the path length. This is enough to conclude the proof.
\end{proof}
